On Identifiability in Transformers

In this paper we delve deep in the Transformer architecture by investigating two of its core components: self-attention and contextual embeddings. In particular, we study the identifiability of attention weights and token embeddings, and the aggregation of context into hidden tokens. We show that, for sequences longer than the attention head dimension, attention weights are not identifiable. We propose effective attention as a complementary tool for improving explanatory interpretations based on attention. Furthermore, we show that input tokens retain to a large degree their identity across the model. We also find evidence suggesting that identity information is mainly encoded in the angle of the embeddings and gradually decreases with depth. Finally, we demonstrate strong mixing of input information in the generation of contextual embeddings by means of a novel quantification method based on gradient attribution. Overall, we show that self-attention distributions are not directly interpretable and present tools to better understand and further investigate Transformer models.

==> token_classification_experiments/rebuttal_plots/GeneralizingAcrossLayers/AllLayers/TokenIdentity_GeneralizeAcrossLayers_LINEAR_COSINE_AllLayers_10FoldCV.tex <==
% This file was created by tikzplotlib v0.8.2.
\begin{tikzpicture}

\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}
\definecolor{color8}{rgb}{0.0901960784313725,0.745098039215686,0.811764705882353}
\definecolor{color6}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color7}{rgb}{0.737254901960784,0.741176470588235,0.133333333333333}

\begin{axis}[
legend cell align={left},
legend columns = 3,
legend style={at={(0.0,0.0)}, anchor=south west, draw=white!80.0!black},
tick align=outside,
tick pos=both,
x grid style={lightgray!92.02614379084967!black},
xlabel={Layer},
xmajorgrids,
width = 0.9\linewidth,
height = \tokenClassifierPlotHeightAppendix,
xmin=0.45, xmax=12.55,
xtick style={color=black},
y grid style={lightgray!92.02614379084967!black},
ylabel={Identifiability Rate},
ymajorgrids,
ymin=0.4, ymax=1.04002459268368,
ytick style={color=black}
]
\addplot [thick, color0]
table {%
1 1
2 1
3 0.981943658370596
4 0.974384512625004
5 0.967806366904788
6 0.95981816347002
7 0.954210191049799
8 0.933868968553002
9 0.89102516263228
10 0.812343264286084
11 0.675274297049946
12 0.685153644930376
};
\addlegendentry{l=1}
\addplot [thick, color1]
table {%
1 1
2 1
3 0.986030526107583
4 0.976692311459636
5 0.963624782207157
6 0.954828386970724
7 0.945201488124362
8 0.919037633634487
9 0.879474574070274
10 0.833273056202626
11 0.730806073556531
12 0.633365787997887
};
\addlegendentry{l=2}
\addplot [thick, color2]
table {%
1 1
2 1
3 1
4 0.993895214558892
5 0.978635481494487
6 0.958406715428431
7 0.939081796779943
8 0.902877553115948
9 0.86258540287932
10 0.822241557627221
11 0.729856152823054
12 0.644893682675023
};
\addlegendentry{l=3}
\addplot [thick, color3]
table {%
1 1
2 1
3 0.999770735965174
4 0.999954022988506
5 0.994391558249252
6 0.977157600639408
7 0.964980298931841
8 0.932257825939553
9 0.895843787132808
10 0.849156008818118
11 0.773511150105568
12 0.729352365383665
};
\addlegendentry{l=4}
\addplot [thick, color4]
table {%
1 0.999952380952381
2 0.999859696560012
3 0.9977107755796
4 0.99880610631942
5 0.998762929557688
6 0.994022345725518
7 0.982562011612471
8 0.971058731123065
9 0.919368328111199
10 0.865252875057741
11 0.806467226828227
12 0.763972078594469
};
\addlegendentry{l=5}
\addplot [thick, color5]
table {%
1 0.997509973478275
2 0.999172382880112
3 0.995202567379097
4 0.994312859244359
5 0.993978270232952
6 0.995661791087932
7 0.989965625665474
8 0.981032771467164
9 0.934871552377645
10 0.876374432850787
11 0.821774222675968
12 0.773986982968302
};
\addlegendentry{l=6}
\addplot [thick, color6]
table {%
1 0.991961368293255
2 0.998815048996014
3 0.991189807001499
4 0.990935623105355
5 0.987997112937912
6 0.988791208802835
7 0.993188518346724
8 0.986430999330965
9 0.957313982710782
10 0.892487037412552
11 0.828898578302189
12 0.760642858783467
};
\addlegendentry{l=7}
\addplot [thick, gray!99.6078431372549!black]
table {%
1 0.980197867971103
2 0.997152344531895
3 0.990749715147209
4 0.991286613264189
5 0.99027679392128
6 0.989732134320758
7 0.990598296353325
8 0.991394288825481
9 0.973665970582077
10 0.902727553565982
11 0.82906882171052
12 0.731629959302344
};
\addlegendentry{l=8}
\addplot [thick, color7]
table {%
1 0.985444136064918
2 0.998206067422752
3 0.98463305279027
4 0.982967428439099
5 0.979787475541485
6 0.977717210940893
7 0.97722867205833
8 0.982577199782243
9 0.987081704812959
10 0.926088215608643
11 0.873033814600403
12 0.767443382287434
};
\addlegendentry{l=9}
\addplot [thick, color8]
table {%
1 0.994130875173655
2 0.994186231926764
3 0.986714705465324
4 0.980940170329605
5 0.979955840961609
6 0.978485715806464
7 0.976501252657776
8 0.978867859759392
9 0.982226536851093
10 0.97830420743293
11 0.915970599845455
12 0.805741932550573
};
\addlegendentry{l=10}
\addplot [thick, color0]
table {%
1 0.991954410179278
2 0.993359342682405
3 0.979693386659757
4 0.976592349902883
5 0.976372578990465
6 0.973976793098691
7 0.971681246854108
8 0.967950966808659
9 0.957353785067388
10 0.924814518843242
11 0.953920470832959
12 0.837012492127621
};
\addlegendentry{l=11}
\addplot [thick, color1]
table {%
1 0.975025294522085
2 0.984020283882439
3 0.977045565463492
4 0.976195811608137
5 0.975158005152879
6 0.973111934434619
7 0.971321194413633
8 0.966590231835631
9 0.952739332037229
10 0.922344687457931
11 0.916836991108777
12 0.935090715445356
};
\addlegendentry{l=12}
\end{axis}

\end{tikzpicture}

==> token_classification_experiments/rebuttal_plots/GeneralizingAcrossLayers/AllLayers/TokenIdentity_GeneralizeAcrossLayers_LINEAR_L2_AllLayers_10FoldCV.tex <==
% This file was created by tikzplotlib v0.8.2.
\begin{tikzpicture}

\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}
\definecolor{color8}{rgb}{0.0901960784313725,0.745098039215686,0.811764705882353}
\definecolor{color6}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color7}{rgb}{0.737254901960784,0.741176470588235,0.133333333333333}

\begin{axis}[
legend cell align={left},
legend columns = 3,
legend style={at={(0.0,0.0)}, anchor=south west, draw=white!80.0!black},
tick align=outside,
tick pos=both,
x grid style={lightgray!92.02614379084967!black},
xlabel={Layer},
xmajorgrids,
width = 0.9\linewidth,
height = \tokenClassifierPlotHeightAppendix,
xmin=0.45, xmax=12.55,
xtick style={color=black},
y grid style={lightgray!92.02614379084967!black},
ylabel={Identifiability Rate},
ymajorgrids,
ymin=0.1, ymax=1.04002459268368,
ytick style={color=black}
]
\addplot [thick, color0]
table {%
1 1
2 0.999726814348332
3 0.989093844709141
4 0.975700927774565
5 0.957959105296981
6 0.922510134703363
7 0.852650716657109
8 0.659824843949406
9 0.484209097553923
10 0.362254122466812
11 0.209052902386952
12 0.19668822789023
};
\addlegendentry{l=1}
\addplot [thick, color1]
table {%
1 1
2 1
3 0.98143013895391
4 0.973139484146228
5 0.955892315981708
6 0.922442885548578
7 0.817538163412863
8 0.535165743575084
9 0.399621095650376
10 0.343111760775686
11 0.289053603873071
12 0.204191544529451
};
\addlegendentry{l=2}
\addplot [thick, color2]
table {%
1 1
2 1
3 0.999356624031546
4 0.9794656689338
5 0.966827936588187
6 0.943590313927984
7 0.891451274203733
8 0.721836557774024
9 0.565362348224097
10 0.458293499153596
11 0.359355722230753
12 0.250145962584927
};
\addlegendentry{l=3}
\addplot [thick, color3]
table {%
1 1
2 1
3 0.988208354731355
4 0.988529030161586
5 0.981231745486848
6 0.964255507391039
7 0.886642001709122
8 0.676876536748488
9 0.515705801183822
10 0.464549003659677
11 0.444801684658714
12 0.308980596225198
};
\addlegendentry{l=4}
\addplot [thick, color4]
table {%
1 0.999956178790535
2 0.999956178790535
3 0.985092375682094
4 0.985963275882784
5 0.982133848038725
6 0.967020828276189
7 0.894156678093572
8 0.691370659193164
9 0.552929191811369
10 0.502836676060805
11 0.50332715033362
12 0.35497807716616
};
\addlegendentry{l=5}
\addplot [thick, color5]
table {%
1 0.983249084858693
2 0.99853309164389
3 0.986219952888185
4 0.982850400783855
5 0.978249071053975
6 0.969408141541138
7 0.919313117411774
8 0.780124005176059
9 0.648464973236009
10 0.59641847602442
11 0.57675383105206
12 0.389117095636526
};
\addlegendentry{l=6}
\addplot [thick, color6]
table {%
1 0.980842349345611
2 0.99281901737578
3 0.98405305151951
4 0.981740965054439
5 0.975794332472677
6 0.969754540899875
7 0.945181491127472
8 0.848291474486706
9 0.745721487451837
10 0.675213141880607
11 0.629185527215802
12 0.428740521901944
};
\addlegendentry{l=7}
\addplot [thick, gray!99.6078431372549!black]
table {%
1 0.979774746188166
2 0.980369718586304
3 0.97179205258229
4 0.981757459882525
5 0.977641353379996
6 0.972818217476398
7 0.960825161390245
8 0.923786909997445
9 0.850568410617843
10 0.758205309784779
11 0.697215182310111
12 0.479446363643788
};
\addlegendentry{l=8}
\addplot [thick, color7]
table {%
1 0.980996659542755
2 0.992277713724767
3 0.980406678207313
4 0.978401667581742
5 0.976417022023932
6 0.972038970818423
7 0.963106852802156
8 0.935882124124389
9 0.893832736959279
10 0.836294224986639
11 0.769375957365563
12 0.524078778128612
};
\addlegendentry{l=9}
\addplot [thick, color8]
table {%
1 0.973164519039182
2 0.992194905760314
3 0.974417700045741
4 0.969388980529172
5 0.96572526867352
6 0.95784626867458
7 0.944668244053577
8 0.908220987331519
9 0.858453323668365
10 0.815359373320691
11 0.772371542686037
12 0.450903129359065
};
\addlegendentry{l=10}
\addplot [thick, color0]
table {%
1 0.958287529256427
2 0.984423806659397
3 0.965408687918805
4 0.9578804184915
5 0.960336249206783
6 0.950756935985801
7 0.940853031630971
8 0.897850159877526
9 0.837443347778777
10 0.783668869178028
11 0.769246666937309
12 0.491147115231167
};
\addlegendentry{l=11}
\addplot [thick, color1]
table {%
1 0.968196254455928
2 0.974226115480827
3 0.960936808447354
4 0.968928665673379
5 0.96462086899595
6 0.961419660223068
7 0.954781631614552
8 0.94083327650245
9 0.909421262886574
10 0.883029241253765
11 0.865762029765831
12 0.733504362659746
};
\addlegendentry{l=12}
\end{axis}

\end{tikzpicture}

==> token_classification_experiments/rebuttal_plots/GeneralizingAcrossLayers/AllLayers/TokenIdentity_GeneralizeAcrossLayers_MLP_COSINE_AllLayers_10FoldCV.tex <==
% This file was created by tikzplotlib v0.8.2.
\begin{tikzpicture}

\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}
\definecolor{color8}{rgb}{0.0901960784313725,0.745098039215686,0.811764705882353}
\definecolor{color6}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color7}{rgb}{0.737254901960784,0.741176470588235,0.133333333333333}

\begin{axis}[
legend cell align={left},
legend columns = 3,
legend style={at={(0.0,0.0)}, anchor=south west, draw=white!80.0!black},
tick align=outside,
tick pos=both,
x grid style={lightgray!92.02614379084967!black},
xlabel={Layer},
xmajorgrids,
width = 0.9\linewidth,
height = \tokenClassifierPlotHeightAppendix,
xmin=0.45, xmax=12.55,
xtick style={color=black},
y grid style={lightgray!92.02614379084967!black},
ylabel={Identifiability Rate},
ymajorgrids,
ymin=0.4, ymax=1.04002459268368,
ytick style={color=black}
]
\addplot [thick, color0]
table {%
1 1
2 1
3 0.983895003127577
4 0.976827502966948
5 0.966528509868508
6 0.953251584362906
7 0.938834620369968
8 0.896512671099973
9 0.815522901101511
10 0.68915871014054
11 0.473397532096209
12 0.587079082232505
};
\addlegendentry{l=1}
\addplot [thick, color1]
table {%
1 1
2 1
3 0.984765451745837
4 0.975600256801532
5 0.963278145485741
6 0.949279868478737
7 0.934318798577009
8 0.900936055578879
9 0.837573425935652
10 0.75915373721932
11 0.617887109389202
12 0.59782833849335
};
\addlegendentry{l=2}
\addplot [thick, color2]
table {%
1 1
2 0.999953183520599
3 1
4 0.987960724626471
5 0.970916625948502
6 0.947575276104365
7 0.923062075084206
8 0.891789780747246
9 0.84041246478579
10 0.782543743244484
11 0.636315182161428
12 0.598393971032451
};
\addlegendentry{l=3}
\addplot [thick, color3]
table {%
1 0.999910117067826
2 0.999909362311134
3 0.999495144437738
4 0.999953938277292
5 0.992817027004021
6 0.978484515823462
7 0.96289515464085
8 0.94008100334378
9 0.882954057903121
10 0.811822178257549
11 0.691770792220177
12 0.662178314771371
};
\addlegendentry{l=4}
\addplot [thick, color4]
table {%
1 0.999404548657016
2 0.999498870417258
3 0.998210363059627
4 0.999322081621475
5 0.999175907161884
6 0.99524942817189
7 0.983618396923539
8 0.96758076452406
9 0.915331573481732
10 0.844872032316305
11 0.750374974437899
12 0.715878626676904
};
\addlegendentry{l=5}
\addplot [thick, color5]
table {%
1 0.997835359327088
2 0.998026163714948
3 0.99650522994931
4 0.997828197935477
5 0.997185465816785
6 0.9972688109081
7 0.991930328948876
8 0.979167909127594
9 0.940269430023697
10 0.855129445410211
11 0.765805377961985
12 0.706593187188366
};
\addlegendentry{l=6}
\addplot [thick, color6]
table {%
1 0.985044172832014
2 0.994090328884317
3 0.993571932992627
4 0.992476272265737
5 0.988391113644336
6 0.99273484458203
7 0.995173666029578
8 0.987501698816576
9 0.952800020501488
10 0.893756747263587
11 0.805613899467241
12 0.750624822552533
};
\addlegendentry{l=7}
\addplot [thick, gray!99.6078431372549!black]
table {%
1 0.962871127210653
2 0.976132436685842
3 0.979270028790288
4 0.982510403401087
5 0.982802422233122
6 0.981781243135085
7 0.987898905907006
8 0.992914838907562
9 0.971521925137461
10 0.903044534831481
11 0.826736044069754
12 0.753479082333096
};
\addlegendentry{l=8}
\addplot [thick, color7]
table {%
1 0.960701217075554
2 0.979455290679498
3 0.972895183928574
4 0.974745672906381
5 0.974819931050398
6 0.975315941030371
7 0.975790414877696
8 0.983081039297162
9 0.987894662673644
10 0.939689657355864
11 0.873454632593301
12 0.79510456038586
};
\addlegendentry{l=9}
\addplot [thick, color8]
table {%
1 0.970504002817262
2 0.973803143950763
3 0.968996484241554
4 0.967191196965653
5 0.969640509404045
6 0.969653791514039
7 0.968139618589185
8 0.968705578646738
9 0.968035773275465
10 0.977532836990608
11 0.903444898059092
12 0.82348733577375
};
\addlegendentry{l=10}
\addplot [thick, color0]
table {%
1 0.940155830381112
2 0.960644620847632
3 0.961584613452446
4 0.965455406583045
5 0.968532365143078
6 0.963228818743349
7 0.956643291482633
8 0.951434443975563
9 0.942840134011846
10 0.918567646389356
11 0.950810652608518
12 0.844885515860979
};
\addlegendentry{l=11}
\addplot [thick, color1]
table {%
1 0.934487222499449
2 0.949651009067318
3 0.951605932620895
4 0.961367770534158
5 0.961920857524043
6 0.957558084972196
7 0.952245011470002
8 0.945250995427592
9 0.935656080577058
10 0.904490642372089
11 0.899541741496457
12 0.93746665754491
};
\addlegendentry{l=12}
\end{axis}

\end{tikzpicture}

==> token_classification_experiments/rebuttal_plots/GeneralizingAcrossLayers/AllLayers/TokenIdentity_GeneralizeAcrossLayers_MLP_L2_AllLayers_10FoldCV.tex <==
% This file was created by tikzplotlib v0.8.2.
\begin{tikzpicture}

\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}
\definecolor{color8}{rgb}{0.0901960784313725,0.745098039215686,0.811764705882353}
\definecolor{color6}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color7}{rgb}{0.737254901960784,0.741176470588235,0.133333333333333}

\begin{axis}[
legend cell align={left},
legend columns = 3,
legend style={at={(0.0,0.0)}, anchor=south west, draw=white!80.0!black},
tick align=outside,
tick pos=both,
x grid style={lightgray!92.02614379084967!black},
xlabel={Layer},
xmajorgrids,
width = 0.9\linewidth,
height = \tokenClassifierPlotHeightAppendix,
xmin=0.45, xmax=12.55,
xtick style={color=black},
y grid style={lightgray!92.02614379084967!black},
ylabel={Identifiability Rate},
ymajorgrids,
ymin=0.1, ymax=1.04002459268368,
ytick style={color=black}
]
\addplot [thick, color0]
table {%
1 1
2 1
3 0.985910148581023
4 0.976396503579664
5 0.953589427343301
6 0.913010835913399
7 0.825907104482371
8 0.633233907287893
9 0.439533614166262
10 0.312296434946768
11 0.215492646657393
12 0.135300457001496
};
\addlegendentry{l=1}
\addplot [thick, color1]
table {%
1 1
2 1
3 0.984006096175556
4 0.973990014633421
5 0.955588474556834
6 0.92125006708979
7 0.836231616160124
8 0.616995668819116
9 0.444818488404442
10 0.351872432121536
11 0.269466994266809
12 0.160549572881785
};
\addlegendentry{l=2}
\addplot [thick, color2]
table {%
1 1
2 1
3 0.999954022988506
4 0.983537339854366
5 0.963598251159782
6 0.935480394800203
7 0.87008309692983
8 0.681255977216454
9 0.519184129007174
10 0.402798781435132
11 0.317930490878664
12 0.190150125641527
};
\addlegendentry{l=3}
\addplot [thick, color3]
table {%
1 0.999907706506691
2 0.999907706506691
3 0.993364930465008
4 0.998337497859689
5 0.993532141793296
6 0.974912243971907
7 0.889422116620501
8 0.678163177685255
9 0.505840734173575
10 0.433426057754229
11 0.399007135868294
12 0.260750780039506
};
\addlegendentry{l=4}
\addplot [thick, color4]
table {%
1 0.999728660902715
2 0.9997260221759
3 0.990030455094563
4 0.991348090442222
5 0.988993050279387
6 0.976013397545902
7 0.921555923606698
8 0.764366628702398
9 0.621299472660879
10 0.52658883655958
11 0.489548485662144
12 0.321026025757387
};
\addlegendentry{l=5}
\addplot [thick, color5]
table {%
1 0.980028814775755
2 0.984134997590195
3 0.986953573318726
4 0.986729059384
5 0.982414837650249
6 0.978333735263727
7 0.948912738603396
8 0.865564809378042
9 0.748055978035151
10 0.637029401413874
11 0.577605746347276
12 0.379312981071257
};
\addlegendentry{l=6}
\addplot [thick, color6]
table {%
1 0.977046674411624
2 0.978208103766203
3 0.974898359192099
4 0.981121977267284
5 0.979072072681306
6 0.972428546510614
7 0.966876970752076
8 0.910074682646726
9 0.815978659236634
10 0.715551665507074
11 0.642334850807429
12 0.43698227139608
};
\addlegendentry{l=7}
\addplot [thick, gray!99.6078431372549!black]
table {%
1 0.972248767406851
2 0.973882898579723
3 0.964394162588241
4 0.975697365231077
5 0.972529238794027
6 0.96914146777654
7 0.967967896486177
8 0.952188316538214
9 0.886851234207733
10 0.781543962868472
11 0.70209236324745
12 0.494697675651548
};
\addlegendentry{l=8}
\addplot [thick, color7]
table {%
1 0.96994413852348
2 0.973071155307252
3 0.959800477355561
4 0.971386218587184
5 0.971458814720048
6 0.967621661665195
7 0.962215922410701
8 0.951072947677891
9 0.928904896240752
10 0.843504159314813
11 0.782647528125424
12 0.539412537835118
};
\addlegendentry{l=9}
\addplot [thick, color8]
table {%
1 0.798832955006941
2 0.847814435799079
3 0.81005529397855
4 0.750005459668649
5 0.734374470651723
6 0.813518059110229
7 0.855375097709028
8 0.880373054317634
9 0.879522865357993
10 0.881180751898194
11 0.81076516911077
12 0.541271412042167
};
\addlegendentry{l=10}
\addplot [thick, color0]
table {%
1 0.891105445348839
2 0.934295374154055
3 0.92632648974526
4 0.938104159586653
5 0.94501250372943
6 0.946512818274902
7 0.941867822542513
8 0.931130605370299
9 0.904318134154977
10 0.84204839807607
11 0.824554749419401
12 0.565664521219615
};
\addlegendentry{l=11}
\addplot [thick, color1]
table {%
1 0.940891346460087
2 0.959542438325255
3 0.943592012192097
4 0.958540474709334
5 0.963826369002099
6 0.959675540291015
7 0.9560020417769
8 0.942280863122082
9 0.924548959171993
10 0.900520935548688
11 0.8882516646736
12 0.822846188668629
};
\addlegendentry{l=12}
\end{axis}

\end{tikzpicture}
